Analyzing constrained LLM through PDFA-learning

We define a congruence that copes with null next-symbol probabilities that arise when the output of a language model is constrained by some means during text generation. We develop an algorithm for efficiently learning the quotient with respect to this congruence and evaluate it on case studies for analyzing statistical properties of LLM.

==> algorithm_old.tex <==
\subsection{Omit-zero}\label{ssec:algorithm}

Based on the theoretical results of Sec.~\ref{sec:lmodels}, we develop an algorithm called \textbf{Omit-Zero}, to learn \indist-minimal PDFA. The algorithm is

\input{assets/algorithms/quant}
%
\noindent
a variant of \QuaNT~(\cite{DBLP:conf/icgi/MayrYCPV23}) that differs in specific steps indicated with boxes in Alg~\ref{alg:quant}.
%
For lack of space, we focus on these. 
%
\textbf{Omit-zero} maintains a tree $\NTree$ whose nodes are strings which are partitioned in two sets, namely, $\AccS\subset\Words$ and $\DisS\subset\Words$ of \emph{access} and \emph{distinguishing} strings, respectively. 
%
\AccS\ is the set of \emph{leafs}. Each $\woru\in\AccS$ is labelled with the distribution $\lmodel(\woru)$. 
%
\DisS\ is the set of non-leaf nodes. 
%
Both \AccS\ and \DisS\ contain \emptyW, which is also the root and a leaf of \NTree.
%
Arcs in \NTree\ are labeled with classes in $\cla{\ProbT}$. 
Every outgoing arc from a non-leaf node is labeled with a different class.  
%
For every $\woru\neq\woru' \in \AccS$, the lowest common ancestor of \woru\ and $\woru'$ in \NTree, $\worw=\lca(\woru, \woru')$, is such that $\lmodel(\woru \worw) \neq\lmodel(\woru' \worw)$.
%
A difference with \QuaNT\ is that we require \NTree\ to satisfy the following properties for all $\woru\in\AccS$:
\begin{align}
    & \isdef{\lmodel}(\woru)=1 \label{req:all_leafs_defined} \\ 
    & \forall\worw\in\pathT_{\woru}.\ \worw\neq\emptyW \implies \worw_1\in\supp(\lmodel(\woru)) \label{req:first_symbol_defined}
\end{align}
where $\pathT_{\woru} \subseteq \DisS$ is the path of distinguishing strings from the root to the leaf $\woru$.
%
Notice that Req.~\ref{req:all_leafs_defined} implies there is no leaf for the class \isundef\ of undefined strings.
%
\textbf{Omit-Zero} \build\ is different to \QuaNT\ in the way transitions are added. For all $\woru\in\AccS$ and $\symb\in\Symb$:
%
\begin{align}\label{omit_zero_build}
\tra(\sta_{\woru}, \symb) &\eqdef 
\begin{cases}
\sta_{\woru'} & \symb\in\supp(\lmodel(\woru)),\ \woru' = \sift(\woru\symb) \\ 
\qhole & \textrm{otherwise}
\end{cases}
\end{align}
%
If \EQ\ returns a counter example $\ce$, i.e, $\lmodel(\ce)\neq\Aut(\ce)$, it is required to be defined in \Aut:
\begin{align}\label{req:ce_defined}
\forall\ce=\EQ(\Aut,\Stasim)\neq\bot.\ \isdef{\Aut}(\ce)=1
\end{align}
%
Let $\lmodel(\ce)\neq\Aut(\ce)$. By Req.~\ref{req:ce_defined} and Prop.~\ref{prop:counterexample}, there is some $\ce_{<j}\in\pref(\ce)$ such that 
%
$\isdef{\lmodel}(\ce_{<j})=1$, $\lmodel(\ce_{<j})\neq\Aut(\ce_{<j})$ and for all $i<j$, $\lmodel(\ce_{<i})=\Aut(\ce_{<i})$.

\textsf{InitializeTree} creates the first instance of \NTree, adding \emptyW\ to \DisS\ as root and as leaf to \AccS, which satisfies $\isdef{\lmodel}(\emptyW)$. \QuaNT\ adds \ce\ to \AccS\ which may not be defined. In contrast, \textbf{Omit-Zero} adds $\ce_{<j}$ to \AccS. 
%
Function \update\ only adds $\ce_{<j}$ to \AccS\ at each call. 
%
The other operation that could add a leaf to \AccS\ is \textsf{sift-update}, called by \sift\ inside \build\ with $\woru\symb$, where $\woru\in\AccS$ and $\symb\in\supp(\lmodel(\woru))$ (Req.~\ref{req:first_symbol_defined}), thus satisfying $\isdef{\lmodel}(\woru\sigma)$.
%
Therefore:
%
\begin{prop}\label{prop:leafs_defined}
\text{\rm\bf Omit-Zero} ensures Req.~\ref{req:all_leafs_defined}. 
\end{prop}
%
The only operation that adds a string $\worw\neq\emptyW$ to \DisS\ is \update, with $\worw=\ce_j\worw'=\lca(\woru,\ce_{<j})$, for some $\woru$ that was already in \AccS, $\ce_j\in\supp(\woru)$, and $\lmodel(\woru)=\lmodel(\ce_{<j})$ (see definition of \sift\ in~\cite{DBLP:conf/icgi/MayrYCPV23}). By~\ref{prop:leafs_defined}, $\isdef{\lmodel}(\woru)=\isdef{\lmodel}(\ce_{<j})=1$. Hence, $\ce_j\in\supp(\ce_{<j})$.

\textcolor{magenta}{STOP}



Prop.~\ref{prop:counterexample} enables sampling strings from the hypothesis when using oracles.


\textcolor{red}{
Here, we visit \QuaNT, the state of the art active learning algorithm for learning PDFA presented in~\cite{DBLP:conf/icgi/MayrYCPV23}, 
where it is empirically shown that active learning PDFA modulo an equivalent relationship in the probability simplex is not only feasible but helps reduce the output hypothesis size. And then propose an extension that we will call \textbf{Omit-Zero} algorithm, which steps on properties of $\indist_\Stasim$  to make the algorithm more efficient.
%
%In contrast to \cite{introduction_to_computational_learning_theory} and \cite{ttt} which build a binary tree, our algorithm handles general trees with arbitrary degree, similar to~\cite{isberner_thesis} for Mealy machines and \cite{Drewes2011} for weighted tree automata.
Both algorithms make use of the same structures, however they differ in specific steps of the process. For simplicity we will explain both algorithms at the same time and make clarifications for the steps where they diverge.
%
}
A tree $\NTree$ maintains a set $\AccS\subset\Words$ of access strings and a set $\DisS\subset\Words$ of distinguishing strings. 
%
Each $\woru\in\AccS$ is bound to a unique leaf in \NTree\ labeled with \MQ(\woru). 
%
Every inner node is labeled with a string $\worw\in\DisS$. 
%
The empty word \emptyW\ belongs to both \AccS\ and \DisS. The root of \NTree\ is labeled with \emptyW. Also, there is a leaf for \emptyW.
%
Arcs in \NTree\ are labeled with classes in $\cla{\ProbT}$. 
Every outgoing arc from an inner node is labeled with a different class.  
%
%
%
Strings in \AccS\ and \DisS\ are connected as follows: for every pair of distinct strings $\woru, \woru' \in \AccS$, the string $\worw\in\DisS$ which is the lowest common ancestor of \woru\ and $\woru'$ in \NTree, denoted $\lca(\woru, \woru')$, is such that $\lmodel(\woru \worw) \neq_{\Stasim}\lmodel(\woru' \worw)$.
%
Therefore, $\woru \not\indist_{\Stasim} \woru'$. 
%
We define $\acctocla{_\NTree} : \AccS \ra \ccla{\Words}$, with $\acctocla{_\NTree}(\woru) = \ccla{\woru}$.
Hence, $\acctocla{_\NTree}$ is one-to-one.

%
%If \Stasim\ induces an infinite partition of \Psimplex(\SymbT), the degree of a node may be unbounded. Indeed, it may be infinite if \ccla{\Words} is infinite.
%
%Notice that this does not occur for non-binary trees used for Mealy machines (\cite{isberner_thesis}).
%
%We will come back to this issue later (in~\ref{ssec:stopping}) after we discuss the learning algorithm.

%
%Fig.~\ref{fig:n_ary_tree_example} shows the trees corresponding to the examples in Fig.~\ref{fig:quotientExample}. 
%
%For $=_\quantp$, with $\quantp = 2$, the leafs of the tree in Fig.~\ref{fig:n_ary_tree_example}(a) correspond to the states of the PDFA of Fig.~\ref{fig:quotientExample}(a), identified with their associated access strings: $\AccS = \{\emptyW, 1, 11, 110, 111\}$.
%
%Every leaf is labeled with the probability distribution of the state.
%
%Tree arcs are labeled with quantization classes, represented with their partition indexes.
%
%For instance, $(1, 0, 0)$ corresponds to the quantization class $(\quanti_{2}^1, \quanti_{2}^0, \quanti_{2}^0)$, where the first coordinate corresponds to the symbol $0$, the second to $1$, and the third to \terminal.
%
%The root \emptyW\ of the tree has an arc for each one of the classes in which quantization partitions the set of probability distributions of the states of the PDFA.
%
%In the example, there are two, namely $(0,0,0)$ and $(0,0,1)$.
%
%\input{assets/pdfa/nary_tree_4}
%
%The tree explains that the five states are not $\indist_\quantp$-equivalent.
%
%Indeed, even if there are states with $=_\quantp$-equivalent distributions, like for example $\sta_0$ and $\sta_1$, the tree shows how the set $\DisS=\{\emptyW,0,1,11\}$ distinguishes them: $\policyW(q_{0}, 11) \in (0,0,0)$ and $\policyW(q_{1}, 11)\in (0,0,1)$.
%
%Fig.~\ref{fig:n_ary_tree_example}(b) corresponds to the PDFA of Fig.~\ref{fig:quotientExample}(b) obtained with \rank.
%
%In this case we label the classes by their ranking, for example $\pdist_0$ ranks first the symbol $0$, second the symbol $1$ and third the symbol \terminal, so it belongs to the class labeled $(0,1,\terminal)$.
%
%Here, $\AccS = \{\emptyW, 1, 11, 111\}$ and $\DisS=\{\emptyW\}$, respectively.
%
%Fig.~\ref{fig:n_ary_tree_example}(c) corresponds to the PDFA of Fig.~\ref{fig:quotientExample}(c) obtained with \topr{1}.
%
%In this case we label the classes by their top symbol, for example $\pdist_2$ ranks first the symbol \terminal, so it belongs to the class labeled \terminal.
%
%Also, $\AccS = \{\emptyW, 1, 11\}$ and $\DisS=\{\emptyW\}$. 

%\begin{prop}\label{prop:tree-size}
%There is a one-to-one mapping from \AccS\ to \ccla{\Words}.
%\proof\rm
%Let $\phi_{\NTree} : \AccS \ra \ccla{\Words}$ be such that $\phi_{\NTree}(\woru) \eqdef \ccla{\woru}$.
%For all $\woru\neq\woru'\in\AccS$, $\worw = \lca(\woru, \woru')$ is such that $\lmodel(\woru\worw) \neq_{\Stasim} \lmodel(\woru' \worw)$. 
%Therefore, $\ccla{\woru}\neq\ccla{\woru'}$. Hence, $\phi_{\NTree}$ is one-to-one. \qedhere
%\end{prop}

\NTree\ defines an equivalence $=_{\NTree} \subseteq \Words\times\Words$.
Let $\pathT_{\woru} \subseteq \DisS$ be the set of distinguishing strings in the path from the root to $\woru \in \AccS$:
%
%\begin{align}\label{def:pathT}
%\woru_1 =_{\NTree} \woru_2 
%    &\iffdef \exists \woru\in\AccS.\ \woru_1 =_{\Stasim}^{\pathT_{\woru}} \woru =_{\Stasim}^{\pathT_{\woru}} \woru_2 
%\end{align}
%
%
\begin{align}\label{def:pathT}
\woru_1 =_{\NTree} \woru_2 
    &\iffdef \exists \woru\in\AccS.\ \forall\worw\in\pathT_{\woru}.\
        \lmodel(\woru_1\worw) =_{\Stasim} \lmodel(\woru\worw) =_{\Stasim} \lmodel(\woru_2\worw)
\end{align}
%
If $\worv\in\Words$ is $=_{\NTree}$-equivalent to some $\woru\in\AccS$ then $\worv \not\indist_{\Stasim} \woru'$ for any other access string 
$\woru' \neq \woru$. As a corollary, \worv\ can be $=_{\NTree}$-equivalent to at most one access string in \NTree. 
%
%\begin{prop}\label{prop:tree-class}
%Let $\woru\in\AccS,\ \worv\in\Words,\ \woru =_{\NTree} \worv$.
%$\forall\woru'\in\AccS.\ \woru' \neq \woru \implies \ccla{\worv} \neq \ccla{\woru'}$.
%\proof\rm
%Let $\woru'\in\AccS$, $\woru' \neq \woru$.
%Then, $\lmodel(\woru' \worw) \neq_{\Stasim} \lmodel(\woru \worw)$ for $\worw = \lca(\woru', \woru)$.
%Since \worw\ is an ancestor of \woru, it follows that $\worw\in\pathT_{\woru}$.
%So, by Def.~\ref{def:pathT}, $\woru =_{\NTree} \worv$ implies $\lmodel(\woru \worw) =_{\Stasim} \lmodel(\worv \worw)$. 
%Therefore, $\lmodel(\woru' \worw) \neq_{\Stasim} \lmodel(\worv \worw)$. 
%Hence, $\ccla{\worv} \neq \ccla{\woru'}$. \qedhere
%\end{prop}
%
To find the $=_{\NTree}$-equivalent leaf (if exists) of $\worv$, we define the function \sift($\worv$) as follows. \sift\ starts at the root of \NTree\ and proceeds recursively. If the current node is a leaf $\woru\in\AccS$, it returns \woru. Otherwise, let $\worw\in\DisS$ be the distinguishing string at the current inner node. 
%
If there is an arc labeled $\cla{\MQ(\worv\worw)}$, \sift\ recursively descends through the arc to the subtree. 
%
Otherwise, it means $\MQ(\worv\worw) \neq_{\Stasim} \MQ(\woru\worw)$ for all descendant leafs \woru\ of \worw. In such case, \sift\ updates the tree as follows: it adds $\worv$ to $\AccS$ labeled with $\MQ(\worv)$ and a new arc from \worw\ to \worv\ labeled with $\cla{\MQ(\worv\worw)}$, and it returns \worv.\footnote{\sift\ updates are necessary since arcs are discovered on-the-fly because \cla{\Psimplex(\SymbT)} may be unbounded.} It is important to remark that, in case \sift\ modifies \NTree, only its degree %(maximum number of outgoing arcs at some node) 
can grow but never its depth. 
%
%\begin{prop}\label{prop:tree-sift}
%For all $\worv\in\Words$, $\sift(\worv)$ returns a leaf \woru\ such that $\worv =_{\NTree} \woru$ and $\ccla{\worv} \neq \ccla{\woru'}$ for all leafs 
%$\woru' \neq \woru$. Also, $\sift$ maintains the properties of the (possibly updated) tree.   
%\proof\rm
%Suppose $\sift(\worv)$ returns an existing leaf \woru. It means it recursively traversed the path $\pathT_{\woru}$ from the root to \woru. 
%Then, by Def.~\ref{def:pathT}, $\worv =_{\NTree} \woru$, and by Prop.~\ref{prop:tree-class}, 
%$\forall\woru'\in\AccS.\ \woru' \neq \woru \implies \ccla{\worv} \neq \ccla{\woru'}$.
%
%Suppose $\sift(\worv)$ returns \worv\ after updating the tree. Obviously, $\worv=_{\NTree}\worv$. Now, this case occurs because \sift\ arrives at an inner node with label $\worw\in\DisS$ for which there is no outgoing arc $=_{\Stasim}$-equivalent to $\lmodel(\worv\worw)$. 
%
%Then, $\ccla{\worv} \neq \ccla{\woru'}$ for any descendant leaf $\woru'$ of the current inner node 
%because $\lmodel(\worv\worw) \neq_{\Stasim} \lmodel(\woru'\worw)$, and \sift\ ensures $\worw = \lca(\woru', \worv)$.
%
%Also, $\ccla{\worv} \neq \ccla{\woru'}$ for any other leaf $\woru'$ in the tree because $\lmodel(\worv\worw') \neq_{\Stasim} \lmodel(\woru'\worw')$ 
%for $\worw' = \lca(\woru', \worw)$, and \sift\ guarantees $\worw' = \lca(\woru', \worv)$. 
%
%Therefore, $\ccla{\worv} \neq \ccla{\woru'}$ for all already existing leafs $\woru'$. 
%
%Moreover, the newly updated tree is such that every pair of distinct leafs is distinguished by its lowest common ancestor and so \acctocla\ is one-to-one. \qedhere
%\end{prop}
%
\input{assets/algorithms/quant}
%
Given \NTree, \build\ constructs a PDFA 
$\Aut \eqdef (\Sta, \staI, \policy, \tra)$ where:
% 
%$\Sta \eqdef \reach(\{\sta_\woru \mid \woru \in \AccS \})$
%\footnote{As in \cite{introduction_to_computational_learning_theory} some states may not be reachable. To keep only reachable ones, we start at \qstaI\ and add states provided they are the destination of a transition.} 
$\Sta \eqdef \{\sta_\woru \mid \woru \in \AccS \}$
with $\accstr(\sta_{\woru}) \eqdef \woru$;
%
$\staI \eqdef \sta_\emptyW$; and
%
for all $q_{\woru} \in \Sta$, $\policy(q_{\woru}) \eqdef \lmodel(\woru)$, and 
%
for all $\symb\in\Symb$, $\tra(q_{\woru}, \symb) \eqdef q_{\woru'}$ with $\woru' = \sift(\woru\symb)$.
%
Whenever \sift\ adds a new leaf, it is restarted with the updated tree.
%
\textcolor{red}{
For the \textbf{Omit-Zero} algorithm \build\ differs in how the transitions are added:
For all $\symb\in\Symb$, $\tra(q_{\woru}, \symb) \eqdef q_{\woru'}$ with $\woru' = \sift(\woru\symb)$ if $\symb\in\supp(\woru)$, else $\tra(q_{\woru}, \symb) \eqdef \qhole$.}

%\begin{prop}\label{prop:build}
%1) If \build\ terminates, the output \Aut\ is irreducible. 
%2) If \ccla{\Words} is finite, $|\Sta|$ is bounded by the size of \ccla{\Words}.
%3) If one of \cla{\Psimplex(\SymbT)} or \ccla{\Words} is finite, \build\ terminates.
%\proof\rm
%Since $\phi_{\NTree}$ is one-to-one, $\sta \neq \sta' \implies \sta \not\indist_{\Stasim} \sta'$.
%This implies that, if \build\ terminates, \Aut\ is irreducible, and if \ccla{\Words} is finite, $|\Sta|$ is at most the size of \ccla{\Words} and also, by Prop.~\ref{prop:tree-sift}, \build\ terminates.
%
%If \cla{\Psimplex(\SymbT)} is %finite, the degree of \NTree\ is %bounded by the size of %$\cla{\Psimplex(\SymbT)}$. Since %\sift\ can only make \NTree\ to %grow in width, it follows \build\ %terminates.
%\qedhere
%\end{prop}
%
%If either \cla{\Psimplex(\SymbT)} or \ccla{\Words} is infinite, \NTree\ could grow without bound. We address this issue in~\ref{ssec:stopping}.
%
Assume \Aut\ is constructed. If \NTree\ and \Aut\ agree for some $\worv\in\Words$ but differ in $\worv\symb$ for some $\symb\in\SymbT$ then \ccla{\worv}\ is not a leaf. Moreover, \worv\ and \sift(\worv)\ are not $\indist_{\Stasim}$-equivalent.

%Formally:
%
%\begin{prop}\label{prop:tree-ce}
%Let $\worv\in\Words, \symb\in\Symb$. If $\sift(\worv) = \accstr(\traW(\worv))$ and $\sift(\worv\symb) \neq \accstr(\traW(\worv\symb))$ then 
%(1) $\worv\not\in\AccS$, and 
%(2) $\sift(\worv) \not\indist_{\Stasim} \worv$.
%\proof\rm
%Let $\woru_1 = \sift(\worv)$, $\woru_2 = \sift(\worv\symb)$, $\woru'_2 = \accstr(\traW(\worv\symb))$, and 
%$\worw = \lca(\woru_2, \woru'_2)$. \\
%(1) 
%Suppose $\worv\in\AccS$. 
%By Prop.~\ref{prop:tree-sift}, $\woru_1 = \worv$, and by construction, $\tra(\sta_{\worv}, \symb) = \sta_{\woru_2}$. 
%Besides, $\traW(\worv\symb) = \tra(\traW(\worv),\symb) = \tra(\sta_{\worv},\symb)$. 
%Then, $\traW(\worv\symb) = \sta_{\woru_2}$.
%So, $\woru'_2 = \accstr(\traW(\worv\symb)) = \accstr(\sta_{\woru_2}) = \woru_2$ which contradicts the hypothesis $\woru_2 \neq \woru'_2$. 
%Hence, $\worv\not\in\AccS$. \\
%(2)
%(i) 
%By Prop.~\ref{prop:tree-sift}, $\woru_2 = \sift(\worv\symb)$ implies $\worv\symb =_{\NTree} \woru_2$.
%So, $\lmodel(\worv\symb\worw) =_{\Stasim} \lmodel(\woru_2\worw)$ since $\worw\in\pathT_{\woru_2}$. \\
%(ii) 
%From $\woru_1 = \accstr(\traW(\worv))$ and $\woru'_2 = \accstr(\traW(\worv\symb))$, 
%it follows by construction of \Aut\ that $\woru'_2 = \sift(\woru_1 \symb)$.
%Then, by Prop.~\ref{prop:tree-sift}, $\woru_1\symb =_{\NTree} \woru'_2$.    
%So, $\lmodel(\woru_1\symb\worw) =_{\Stasim} \lmodel(\woru'_2\worw)$ since $\worw\in\pathT_{\woru'_2}$. \\
%
%Therefore, from $\lmodel(\woru_2\worw) \neq_{\Stasim} \lmodel(\woru'_2\worw)$, (i) and (ii) 
%it follows that $\lmodel(\worv\symb\worw) \neq_{\Stasim} \lmodel(\woru_1\symb\worw)$.
%So, $\woru_1 \not\indist_{\Stasim} \worv$.
%Hence, $\sift(\worv) \not\indist_{\Stasim} \worv$.
%\qedhere
%\end{prop}
%
%
Assume \EQ(\Aut) returns a counterexample \ce. 
%
Let $\woru_i = \sift(\ce[i])$ and $\woru'_i = \accstr(\traW(\ce[i]))$.
%
Since $\lmodel(\ce) \neq_{\Stasim} \policyW(\ce)$, there is some $i$ such that $\woru_i \neq \woru'_i$. Let $j$ be the first such index.
Therefore, Prop.~\ref{prop:tree-ce} implies $\ce[j-1] \not\in\AccS$ and $\woru_{j-1} \not\indist_{\Stasim} \ce[j-1]$.
Moreover, $\ce_j\worw$ distinguishes $\woru_{j-1}$ and $\ce[j-1]$ with $\worw = \lca(\woru_j, \woru'_j)$.
%
The procedure \update\ modifies \NTree\ with this new evidence as follows:
%
$\ce[j-1]$ is added to \AccS, and
%
the leaf $\woru_{j-1}$ is replaced by an inner node $\ce_{j}\worw$ and two children, namely $\woru_{j-1}$ and $\ce[j-1]$.
%
\update\ maintains the properties of the tree. 
%
\textcolor{red}{
For the case of \textbf{Omit-Zero} algorithm \EQ\ is also required to return a counter example $\ce$, such that  $\isdef{\Aut}(\ce)=1$.}
%
Algorithm~\ref{alg:quant} sketches the code. It starts creating an initial $\Aut$, with a single state $q_\emptyW$ with a loop for each symbol and probability distribution $\MQ(\emptyW)$.
%
Then, it calls $\EQ(\Aut)$, which either returns $\bot$ and terminates or a counterexample \ce\ triggering the initialization of \NTree. The first instance of \NTree\ has a root \emptyW\ and two children, one labeled \emptyW\ and the other \ce.\textcolor{red}{ For the \textbf{Omit-Zero} algorithm the children \ce\ is substituted by the shortest prefix \ce[j] of \ce\, such that $\lmodel(\ce[j]) \neq_{\Stasim} \policyW(\ce[j])$, in other words, \ce[j] is a counterexample.}
%
In the main loop, Algorithm~\ref{alg:quant} uses \NTree\ to build a PDFA $\Aut$, then calls \EQ(\Aut). If a counterexample is returned, \NTree\ is updated and the loop restarts. Otherwise, it terminates.
%
Algorithm~\ref{alg:quant} learns a \textcolor{orange}{PAC-equivalent PDFA.}\\
\textcolor{violet}{
\begin{prop}%[The shortest prefix of a counterexample in the hypothesis is defined in the target LM]
\label{prop:shortest_prefix_is_defined}
For any $\ce\in\Words$ such that $\isdef{\hAut}(\ce) = 1$ and $\lmodel(\ce)\neq_\Stasim\hAut(\ce)$ then, for $\ce[j]\in\pref(\ce)$ the shortest element such that $\lmodel(\ce[j])\neq_\Stasim\hAut(\ce[j])$ $\implies \isdef{\lmodel}(\ce[j]) = 1$ 
\proof\rm 
By absurd, let us assume $\isdef{\lmodel}(\ce[j]) = 0$.
1) By definition of $\isdef{\lmodel}$ $\exists \woru\symb \in\pref(\ce[j])$ such that $\isdef{\lmodel}(\woru) = 1$ and $\isdef{\lmodel}(\woru\symb) = 0$.
2) By hypothesis $\isdef{\hAut}(\ce) = 1$, then $\isdef{\hAut}(\woru) = 1$ and $\isdef{\hAut}(\woru\symb) = 1$. 
By 1) and 2) $\supp(\lmodel(\woru))\neq\supp(\hAut(\woru))$.
Then $\lmodel(\woru)\neq_\Stasim\hAut(\woru)$ and $|\woru|<|\ce[j]|$. Which contradicts the hypothesis of $\ce[j]$ being the shortest prefix.
\qedhere
\end{prop}
}

\textcolor{violet}{
\begin{prop}[All leafs are defined]\label{prop:leafs_defined}
At every step of the \textbf{Omit-Zero} algorithm, $\forall \accstr\in\AccS , \isdef{\lmodel}(\accstr)=1$. 
\proof\rm 
This can be proved following operations \textit{initializeTree},  \textit{update} and \textit{sift-update}. As those are the ones that add elements to \AccS.
As described before, Initialize adds two elements to \AccS, those are \emptyW\ and \ce[j] the shortest prefix of \ce\ such that \ce[j] is still a counterexample. By definition $\isdef{\lmodel}(\emptyW)=1$. By prop.~\ref{prop:counterexample} and prop.~\ref{prop:shortest_prefix_is_defined}, we have $\isdef{\lmodel}(\ce[j])=1$.
For the case of \textit{update} only one element is added at each call. This element is $\ce[j-1]$ and by prop.~\ref{prop:shortest_prefix_is_defined}\ $\isdef{\lmodel}(\ce[j])=1 \implies \isdef{\lmodel}(\ce[j-1])=1$.
For the \textit{sift-update} operation, the function is only called with $\worw = \woru\sigma$ where $\woru\in\AccS$ and $\sigma\in\supp(\lmodel(\woru))$, thus $\isdef{\lmodel}(\woru\sigma)$.
\qedhere
\end{prop}}

\textcolor{red}{
\begin{prop}[All distinguishing strings are defined by their first symbol]\label{prop:leafs_defined}
At every step of the \textbf{Omit-Zero} algorithm, $\forall \accstr\in\AccS, \forall \worw \in\pathT_{\accstr} \suchthat \worw = \sigma\woru \implies \sigma\in\supp(\accstr)$. 
\proof\rm 
As before, this can be proved following operations that modify \NTree. Those are \textit{initializeTree},  \textit{update} and \textit{sift-update} inside \textit{build}. As those are the ones that either add elements to \AccS\ or to \DisS.
As described before, \textit{initializeTree} adds two elements however $\DisS = {\emptyW}$, and $\emptyW \neq \sigma\woru$.
For the case of \textit{update}, the new inner node is composed by $\ce_j\worw$, by prop.~\ref{prop:shortest_prefix_is_defined}, we have $\isdef{\lmodel}(\ce[j])=1$, which means that for the new leaf $\ce[j-1]$, $\ce_j \in\supp(\lmodel(\ce[j-1]))$. For the other leaf, $\woru_{j-1}$, by definition of sift we have that $\supp(\lmodel(\ce[j-1])) = \supp(\lmodel(\woru_{j-1}) \implies \ce_j \in\supp(\lmodel(\woru_{j-1}))$.
Finally, for the case of \textit{sift-update} inside \textit{build} we have....
\qedhere
\end{prop}
}


\textcolor{orange}{Following propositions are presented for the \textbf{Omit-Zero} version of the algorithm, as their standard counterparts are already proved in \cite{DBLP:conf/icgi/MayrYCPV23}.
}
\textcolor{orange}{
\begin{prop}[Correctness]\label{prop:correctness}
If Algorithm~\ref{alg:quant} terminates, it outputs an irreducible PDFA which is $\indist_{\Stasim}$-equivalent (in the sense of PAC) to \lmodel.
\proof\rm 
Let \Aut\ be the output of Algorithm~\ref{alg:quant}. Then, $\Aut \indist_{\Stasim} \lmodel$ (in the sense of PAC) since \EQ(\Aut) does not return a counterexample. By Prop.~\ref{prop:build}(1), \Aut\ is irreducible.
\qedhere
\end{prop}
%
\begin{prop}[Strict progress]\label{prop:progress}
Let $\Aut_i$ be the PDFA built by Algorithm~\ref{alg:quant} at iteration $i$. If $\EQ(\Aut_i) \neq \bot$ then $\Aut_{i+1}$, if built, has strictly more states than $\Aut_i$.
\proof\rm 
If $\EQ(\Aut_i) \neq \bot$, \update\ adds a new leaf to \NTree. Hence, $|\Sta_{i+1}| > |\Sta_i|$.
\qedhere
\end{prop}
%
\begin{cor}
Algorithm~\ref{alg:quant} always terminates for \Stasim-regular languages. 
%if \ccla{\Words} is finite.
\proof\rm From Prop.~\ref{prop:progress}, Prop.~\ref{prop:build}, Prop.~\ref{prop:congruence_stasim_minimal}, and Prop.~\ref{prop:s_suff_str_traW}.
\end{cor}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> assets/algorithms/initialize_observation_tree.tex <==
%\begin{algorithm}[H]
%    \SetKwInOut{Input}{Input}
%    \SetKwInOut{Output}{Output}
%    \SetKwInOut{Parameter}{Parameter}
    
%    \Input{Counterexample $ce$}
%    \Parameter{Quantization Parameter $\kappa$}
%    \Output{N-ary Observation Tree $T$}
    
%    epsilon_child
    
%    \Return T\;
%    \caption{Initialize-Observation-Tree}
%    \label{alg:init-observation-tree}
%\end{algorithm}
